Verification and Synthesis of Control Barrier Functions

Control systems often must satisfy strict safety requirements over an extended operating lifetime. Control Barrier Functions (CBFs) are a promising recent approach to constructing simple and safe control policies. This paper proposes a framework for verifying that a CBF guarantees safety for all time and synthesizing CBFs with verifiable safety in polynomial control systems. Our approach is to show that safety of CBFs is equivalent to the non-existence of solutions to a family of polynomial equations, and then prove that this nonexistence is equivalent to a pair of sum-of-squares constraints via the Positivstellensatz of algebraic geometry. We develop this Positivstellensatz to verify CBFs, as well as generalization to high-degree systems and multiple CBF constraints. We then propose a set of heuristics for CBF synthesis, including a general alternating-descent heuristic, a specialized approach for compact safe regions, and an approach for convex unsafe regions. Our approach is illustrated on two numerical examples.

==> Formulation.tex <==
\section{Problem Formulation and Solution Approach}
\label{sec:formulation}
This section presents our problem statement, solution approach, and safety proof.

\subsection{System Model and Problem Statement}
\label{subsec:problem-statement}
We consider systems with state $x(t) \in \mathbb{R}^{n}$ and input $u(t) \in \mathbb{R}^{m}$. We consider linear dynamics of the form 
\begin{equation}
\label{eq:dynamics}
\dot{x}(t) = Fx(t) + Gu(t). 
\end{equation}
We assume that the pair $(F,G)$ is controllable. The goal of the system is to satisfy a safety constraint of the form $x(t) \in \mathcal{C}$ for all time $t$. Specifically, we assume that the set $\mathcal{C}$ is encoded as the super-level set of a function $h: \mathbb{R}^{n} \rightarrow \mathbb{R}$, so that 
\begin{equation}
\label{eq:safety-constraint}
\mathcal{C} = \{x : h(x) \geq 0\}, \quad \partial C = \{x: h(x) = 0\}
\end{equation}
 and the safety condition reduces to ensuring that $h(x(t)) \geq 0$ for all time $t$. 

\begin{Definition}
\label{def:viability-kernel}
A vector $x_{0} \in \mathcal{C}$ is in the \emph{viability kernel} of system (\ref{eq:dynamics}) with safety constraint (\ref{eq:safety-constraint}) if there exists a control signal $\{u(t) : t \geq 0\}$ such that $x(t) \in \mathcal{C}$ for all time $t$ when $x(0) = x_{0}$.
\end{Definition}

The problem studied in this paper can be viewed as joint construction of a viability kernel and a control strategy to ensure safety, and is stated formally as follows.

\emph{Problem Studied:} Construct a set $\overline{\mathcal{C}} \subseteq \mathcal{C}$ and a function $\mathcal{U}: \overline{\mathcal{C}} \rightarrow \mathcal{P}(\mathbb{R}^{m})$ such that, if $x(0) \in \overline{\mathcal{C}}$ and $u(t) \in \mathcal{U}(x(t))$ for all time $t$, then $x(t) \in \overline{\mathcal{C}}$ for all time $t$.

Intuitively, the set $\overline{\mathcal{C}}$ is an approximation of the viability kernel. The function $\mathcal{U}(x)$ defines a subset of control inputs corresponding to $x \in \overline{\mathcal{C}}$, so that if $u(t) \in \mathcal{U}(x(t))$ for all time $t$, then safety is satisfied. Hence, safe control policies can be constructed by ensuring that the constraint $u(t) \in \mathcal{U}(x(t))$ is satisfied for all time $t$.

Our approach to constructing control policies is grounded on the concept of \emph{Control Barrier Function}. The function $\overline{h}: \mathbb{R}^{n} \rightarrow \mathbb{R}$ defines a CBF for $\mathcal{C}$ if $\overline{h}(x) \geq 0$ implies that $h(x) \geq 0$ and, for some class-K function $\beta$, 
\begin{equation}
\label{eq:CBF-def}
\sup_{u}{\{\frac{\partial \overline{h}}{\partial x}Fx + \frac{\partial \overline{h}}{\partial x}Gu\}} \geq -\beta(\overline{h}(x)).
\end{equation}
Since $\overline{h}(x) \geq 0$ implies that $h(x) \geq 0$, if $\overline{h}(x(t)) \geq 0$ for all time $t$, then $h(x(t)) \geq 0$ for all time $t$ and safety is satisfied. Furthermore, the constraint (\ref{eq:CBF-def}) ensures that if $\overline{h}(x(t)) = 0$, then $\frac{d}{dt}\overline{h}(x(t)) \geq 0$ and hence the system will never enter the region $\overline{h}(x(t)) < 0$. Hence, these two combined properties of CBFs ensure system safety, as formalized in the following theorem.

\begin{Theorem}[\textbf{*ref Coogan survey}]
\label{theorem:CBF-safety}
If $\overline{h}$ is a control barrier function and $\frac{\partial \overline{h}}{\partial x}(x) \neq 0$ for all $x$ with $\overline{h}(x) = 0$, then any Lipschitz continuous controller satisfying (\ref{eq:CBF-def}) for all time $t$ renders the set $\{\overline{h}(x) \geq 0\}$ safe.
\end{Theorem}

The existence of a CBF is sufficient (\textbf{*give converse also?}) to ensure safety, however, the preceding discussion does not provide an approach to computing a CBF. The ideal case is one in which $h$ itself is a CBF. This is not guaranteed, however, particularly when the system is not fully actuated (i.e., $\mbox{rank}(G) < n$). In Section \ref{subsec:verification}, we give a procedure for checking whether a given function $\overline{h}$ is a CBF. Next, we give a first step towards ensuring safety, beginning with the following observation.

\begin{Lemma}
\label{lemma:coordinate-transform}
Let $P$ be an invertible matrix. Suppose that $\overline{\mathcal{C}}$ is a positive invariant set for the system $(PFP^{-1},PG)$ with constraint function $\mathcal{U}$. Then the set $\overline{\mathcal{C}}^{\prime} = \{x: Px \in \overline{\mathcal{C}}\}$ is positive invariant with constraint function $\mathcal{U}^{\prime} = \mathcal{U}(Px)$.
\end{Lemma}

\textbf{*Need to put proof.} By Lemma \ref{lemma:coordinate-transform}, we assume without loss of generality that the system is in a canonical form with 
\begin{displaymath}
F = \left(
\begin{array}{cc}
F_{11} & F_{12} \\
I_{n-m} & 0 
\end{array}
\right), \quad G = \left(
\begin{array}{c}
I_{m} \\
0
\end{array}
\right)
\end{displaymath}
Any controllable linear system can be put in this form \textbf{*ref Chen's book}. We decompose the system state as $x(t) = (x_{1}(t)^{T} \ x_{2}(t)^{T})^{T}$, where $x_{1}(t)$ denotes the first $m$ entries and $x_{2}(t)$ denotes the remaining $(n-m)$ entries. We write $F_{1} = (F_{11} \ F_{12})$.

 Under this approach, for a function $h$, we have that $\frac{\partial h}{\partial x}Fx + \frac{\partial h}{\partial x}Gu$ can be written as $$\frac{\partial h}{\partial x_{1}}F_{1}x + \frac{\partial h}{\partial x_{1}}u + \frac{\partial h}{\partial x_{2}}F_{2}x.$$ We therefore clearly have that the CBF constraints can be satisfied iff $\frac{\partial h}{\partial x_{2}}F_{2}x \geq 0$ whenever $\frac{\partial h}{\partial x_{1}} = 0$. We can  partition the set $\mathcal{C}$ into two subsets. If $\frac{\partial h}{\partial x_{2}}F_{2}x \geq 0$, then choosing a $u$ that satisfies $$\frac{\partial h}{\partial x_{1}}F_{1}x + \frac{\partial h}{\partial x_{1}}u + \frac{\partial h}{\partial x_{2}}F_{2}x \geq -\beta(h(x)),$$ or $u(t) = 0$ if $\frac{\partial h}{\partial x_{1}} = 0$, is sufficient. If $\frac{\partial h}{\partial x_{2}} < 0$, then we attempt to ensure that $$\frac{\partial h}{\partial x_{2}}F_{2}x \geq -\alpha_{1}(h(x))$$ for some class-K function $\alpha$. 
 
 Generalizing this approach, we define a sequence of sets $\mathcal{C}_{i}$ and CBFs $h_{i}$ as follows. Let $h_{1}(x) = h(x)$ and define $\mathcal{C}_{1}$ by $$\mathcal{C}_{1} = \{\frac{\partial h}{\partial x_{2}}F_{2}x \geq 0 \} \cap \{h(x) \geq 0\}.$$ Proceeding inductively, we let $$h_{i+1}(x) = \frac{\partial h_{i}}{\partial x_{2}}F_{2}x + \alpha_{i}(h_{i}(x)),$$ where $\alpha_{i}$ is a class-K function, and $$\mathcal{C}_{i+1} = \{\frac{\partial h_{i}}{\partial x_{2}}F_{2}x < 0 \} \cap \{\frac{\partial h_{i+1}}{\partial x_{2}}F_{2}x \geq 0\} \cap \left(\bigcap_{j=1}^{i+1}{\{h_{j}(x) \geq 0\}}\right).$$
 
 We have the following safety result.
 \begin{Theorem}
 \label{theorem:general-safety}
 Suppose that there exists $r$ such that there is no $x$ in $\mathcal{C}_{r}$ satisfying $h_{r}(x) = 0$ and $\frac{\partial h_{r}}{\partial x_{1}} = 0$. Then $\bigcup_{i=1}^{r}{\mathcal{C}_{i}}$ is positive invariant under the constraint set 
\begin{displaymath} 
 \mathcal{U}(x) = \left\{
 \begin{array}{ll}
 \frac{\partial h_{i}}{\partial x}(Fx + Gu) \geq -\beta_{i}(x), & \frac{\partial h_{i}}{\partial x_{1}} \neq 0 \\
 \mathbb{R}^{m}, & \frac{\partial h_{i}}{\partial x_{1}} = 0
 \end{array}
 \right.
 \end{displaymath}
 for $x \in \mathcal{C}_{i}$. 
 \end{Theorem}
 
 \begin{proof}
 
 
  %On the other hand, if $\frac{\partial h}{\partial x_{2}}F_{2} x < 0$, then we must ensure that the set 

